Deep learning network to correct axial and coronal eye motion in 3D OCT retinal imaging

Optical Coherence Tomography (OCT) is one of the most important retinal imaging technique. However, involuntary motion artifacts still pose a major challenge in OCT imaging that compromises the quality of downstream analysis, such as retinal layer segmentation and OCT Angiography. We propose deep learning based neural networks to correct axial and coronal motion artifacts in OCT based on a single volumetric scan. The proposed method consists of two fully-convolutional neural networks that predict Z and X dimensional displacement maps sequentially in two stages. The experimental result shows that the proposed method can effectively correct motion artifacts and achieve smaller error than other methods. Specifically, the method can recover the overall curvature of the retina, and can be generalized well to various diseases and resolutions.

==> tables/curvature.tex <==
% result table
\begin{table*}[htb]
% \tabcolsep=0.11cm
    \caption{Quantitative result of different axial motion correction on the test set.}
    \centering
    \begin{tabular}{@{}l@{\hskip6pt}l@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{}}
    \toprule
        \multicolumn{2}{c}{Method} & $\mathrm{MAE_z}$ & $\mathrm{PCC}(\mathbf{V}_\mathrm{dz},\mathbf{V}_\mathrm{GT})$ & $\mathrm{Curv}_x$ & $\mathrm{Dist}_x$ & $\mathrm{Curv}_y$ & $\mathrm{Dist}_y$ & $\mathrm{Dist}_{xy}$  \\
    \midrule % GT
        \multicolumn{2}{@{}l}{Before correction}
        & 22.742 (±20.703)
        & 0.5505 (±0.1492)
        & 1.0020 (±0.0023)
        & -
        & -
        & -
        & -
        \\
        
        \multicolumn{2}{@{}l}{Ground truth}
        & -
        & 1.0000 (±0.0000)
        & 1.0020 (±0.0023)
        & -
        & 1.0013 (±0.0015)
        & -
        & 0.0010 (±0.0013)
        \\
    \midrule % methods
        \multicolumn{2}{@{}l}{Antony et al. \cite{antony2011automated}}
        & 40.530 (±17.118)
        & 0.3517 (±0.1144)
        & 1.0000 (±0.0000)
        & 0.0020 (±0.0023)
        & 1.0000 (±0.0000)
        & 0.0012 (±0.0015)
        & 0.0020 (±0.0023)
        \\
        
        \multicolumn{2}{@{}l}{Montuoro et al. \cite{montuoro2014motion}}
        & 20.543 (±19.853)
        & 0.5666 (±0.1523)
        & \textbf{1.0020} (±0.0023)
        & \textbf{0.0000} (±0.0000)
        & 1.0051 (±0.0081)
        & 0.0040 (±0.0072)
        & 0.0044 (±0.0069)
        \\
        
        \multicolumn{2}{@{}l}{Fu et al. \cite{fu2016eye}}
        & 20.963 (±18.394)
        & 0.5605 (±0.1403)
        & \textbf{1.0020} (±0.0023)
        & \textbf{0.0000} (±0.0000)
        & 1.0048 (±0.0072)
        & 0.0043 (±0.0066)
        & 0.0042 (±0.0064)
        \\
        
        \multicolumn{2}{@{}l}{Spectralis \cite{teussink2019spectralis}}
        & 15.253 (±9.746)
        & 0.6000 (±0.1396)
        & \textbf{1.0020} (±0.0023)
        & \textbf{0.0000} (±0.0000)
        & 1.0003 (±0.0007)
        & 0.0010 (±0.0014)
        & 0.0017 (±0.0020)
        \\
        
    \midrule
        \multirow{2}{*}{Ours (baseline)} 
        & -
        & 13.948 (±10.833)
        & 0.6185 (±0.1124)
        & 1.0017 (±0.0016)
        & 0.0007 (±0.0014)
        & \textbf{1.0013} (±0.0015)
        & 0.0009 (±0.0011)
        & 0.0013 (±0.0014)
        \\
        
        & LS
        & 12.720 (±9.504)
        & 0.6388 (±0.1139)
        & \textbf{1.0020} (±0.0023)
        & \textbf{0.0000} (±0.0000)
        & 1.0016 (±0.0018)
        & 0.0009 (±0.0011)
        & \textbf{0.0012} (±0.0012)
        \\
        
       \multirow{2}{*}{Ours (with seg.)}
        & -
        & 9.102 (±7.972)
        & 0.7150 (±0.0965)
        & 1.0012 (±0.0012)
        & 0.0009 (±0.0018)
        & 1.0009 (±0.0005)
        & 0.0008 (±0.0013)
        & 0.0015 (±0.0021)
        \\
        
        & LS
        & \textbf{8.512} (±8.211)
        & \textbf{0.7277} (±0.1107)
        & \textbf{1.0020} (±0.0023)
        & \textbf{0.0000} (±0.0000)
        & 1.0008 (±0.0005)
        & \textbf{0.0006} (±0.0012)
        & 0.0014 (±0.0019)
        \\
        
    \bottomrule
    \end{tabular}
    \label{tab:moco_z}
\end{table*}


% % result table
% \begin{table*}[htb]
% % \tabcolsep=0.11cm
%     \caption{Quantitative result of different axial motion correction on the test set.}
%     \centering
%     \begin{tabular}{llcccc}
%     \toprule
%         \multicolumn{2}{c}{Method} & $\mathrm{MAE}_z$ & MNMI  & MPCC  \\
%     \midrule % GT
%         \multicolumn{2}{l}{Before correction}
%         & 22.7421 (±20.7032)
%         & 0.5734 (±0.0273) %0.5912 (±0.0323)
%         & 0.6777 (±0.0833)
%         \\
        
%         \multicolumn{2}{l}{Ground truth \cite{potsaid2008ultrahigh}}
%         & -
%         & 0.6097 (±0.0378) %0.5932 (±0.0326)
%         & 0.8556 (±0.0288)
%         \\
%     \midrule % methods
%         \multicolumn{2}{l}{Antony et al. \cite{antony2011automated}}
%         & 19.3896 (±11.5209)
%         & 0.5953 (±0.0344)
%         & 0.8689 (±0.0280)
%         \\
        
%         \multicolumn{2}{l}{Montuoro et al. \cite{montuoro2014motion}}
%         & 20.5433 (±19.8528)
%         & 0.6086 (±0.0367) %0.5923 ($\pm$0.0312)
%         & 0.7812 (±0.0577)
%         \\
        
%         \multicolumn{2}{l}{Fu et al. \cite{fu2016eye}}
%         & 26.6662 (±15.5819)
%         & 0.6053 (±0.0379) %0.5905 ($\pm$0.0313)
%         & 0.8160 (±0.0618)
%         \\
        
%         \multicolumn{2}{l}{Heidelberg \cite{rocholz2018spectralis}}
%         & 21.6630 (±19.7298)
%         & 0.6054 (±0.0370)
%         & 0.8785 (±0.0200)
%         \\
        
%     \midrule
%         \multirow{2}{*}{Our proposed (baseline)} 
%         & -
%         & 13.6755 (±9.6111)
%         & 0.6053 (±0.0384)
%         & 0.7446 (±0.0358)
%         \\
        
%         & LS
%         & 12.9390 (±9.7903)
%         & 0.6070 (±0.0387) %0.5891 (±0.0329)
%         & 0.7842 (±0.0393)
%         \\
        
%       \multirow{2}{*}{Our proposed (with seg.)}
%         & -
%         & 9.2351 (±7.9323)
%         & \textbf{0.6095 (±0.0379)}
%         & 0.8389 (±0.0273)
%         \\
        
%         & LS
%         & \textbf{8.6454} (±8.1501)
%         & 0.6100 (±0.0383) %0.5924 (±0.0327)
%         & \textbf{0.8423 (±0.0271)}
%         \\
        
%     \bottomrule
%     \end{tabular}
%     \label{tab:moco_z}
% \end{table*}

==> tables/disease_hv.tex <==
\begin{table*}[htb]
% \tabcolsep=0.11cm
    \caption{Quantitative result of different motion correction methods on the test set with different diseases.}
    \centering
    % \scriptsize
    \fontsize{7.8}{9}\selectfont
    \begin{tabular*}{\linewidth}{@{}l@{\hskip5pt}l@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{}}
    \toprule
        & & & & \multicolumn{6}{c}{Joint Z + X correction} \\
        \cmidrule(lr){5-10}
    & Metrics & Before correction & GT & Antony et al. \cite{antony2011automated} & Montuoro et al. \cite{montuoro2014motion} & Fu et al. \cite{fu2016eye} & Spectralis \cite{teussink2019spectralis} & Ours (baseline) & Ours (with seg.) \\
\midrule
    All data & MAE$_z$  & 22.742 (20.703) & - & 40.530 (17.118) & 20.543 (19.853) & 20.962 (18.394) & 15.253 (9.746) & 12.720 (9.504) & \textbf{8.5118} (8.211) \\
    & MAE$_x$ & 0.7484 (0.449) & - & 0.7484 (0.449) & 1.8507 (0.544) & 0.8232 (0.414) & - & \textbf{0.7428} (0.440) & 0.7401 (0.440) \\
    & PCC & 0.5505 (0.149) & - & 0.3517 (0.114) & 0.5635 (0.151) & 0.5604 (0.140) & 0.6043 (0.141) & 0.6388 (0.114) & \textbf{0.7277} (0.111) \\
    & Dice & 0.9205 (0.051) & - & 0.9205 (0.051) & 0.7663 (0.070) & 0.9119 (0.046) & - & \textbf{0.9214} (0.049) & 0.9219 (0.049) \\
    & Curv$_x$  & 1.0020 (0.002) & 1.0020 (0.002) & 1.0000 (0.000) & \textbf{1.0020} (0.002) & \textbf{1.0020} (0.002) & \textbf{1.0020} (0.002) & \textbf{1.0020} (0.002) & \textbf{1.0020} (0.002) \\
    & Dist$_x$  & - & - & 0.0020 (0.002) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) \\
    & Curv$_y$  & - & 1.0013 (0.002) & 1.0000 (0.000) & 1.0051 (0.008) & 1.0048 (0.007) & 1.0003 (0.001) & \textbf{1.0016} (0.002) & 1.0008 (0.001) \\
    & Dist$_y$  & - & - & 0.0012 (0.002) & 0.0040 (0.007) & 0.0043 (0.007) & 0.0010 (0.001) & 0.0009 (0.001) & \textbf{0.0006} (0.001) \\
    & Dist$_{xy}$  & - & - & 0.0020 (0.002) & 0.0044 (0.007) & 0.0042 (0.006) & 0.0017 (0.002) & \textbf{0.0012} (0.001) & 0.0014 (0.002) \\
% \midrule
%     All data & MAE$_x$ & 0.7484 (0.449) & - & 0.7484 (0.449) & 1.6152 (0.460) & 0.8185 (0.438) & - & \textbf{0.7406} (0.437) & \textbf{0.7406} (0.437) \\
%     GT Z + X & PCC & 0.9714 (0.019) & - & 0.9714 (0.019) & 0.9506 (0.015) & 0.9693 (0.019) & - & \textbf{0.9716} (0.019) & \textbf{0.9716} (0.019) \\
%     & Dice & 0.9205 (0.051) & - & 0.9205 (0.051) & 0.8191 (0.056) & 0.9127 (0.049) & - & \textbf{0.9218} (0.048) & \textbf{0.9218} (0.048) \\
\midrule
    AMD & MAE$_z$  & 25.752 (21.464) & - & 22.418 (11.606) & 23.237 (19.945) & 26.140 (11.808) & 24.467 (19.712) & 16.516 (11.862) & \textbf{11.827} (11.178) \\
    & MAE$_x$ & 1.0204 (0.225) & - & 1.0204 (0.225) & 2.0829 (0.315) & 1.0651 (0.209) & - & 1.0140 (0.215) & \textbf{1.0102} (0.216) \\
    & PCC & 0.5424 (0.126) & - & 0.3609 (0.151) & 0.5542 (0.135) & 0.5617 (0.094) & 0.5481 (0.112) & 0.6093 (0.113) & \textbf{0.7064} (0.132) \\
    & Dice & 0.8890 (0.035) & - & 0.8890 (0.035) & 0.7408 (0.061) & 0.8843 (0.033) & - & 0.8901 (0.033) & \textbf{0.8909} (0.033) \\
    & Curv$_x$  & 1.0030 (0.003) & 1.0030 (0.003) & 1.0000 (0.000) & \textbf{1.0030} (0.003) & \textbf{1.0030} (0.003) & \textbf{1.0030} (0.003) & \textbf{1.0030} (0.003) & \textbf{1.0030} (0.003) \\
    & Dist$_x$  & - & - & 0.0030 (0.003) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) \\
    & Curv$_y$  & - & 1.0020 (0.002) & 1.0000 (0.000) & 1.0065 (0.010) & 1.0060 (0.006) & 1.0005 (0.001) & \textbf{1.0022} (0.002) & 1.0011 (0.001) \\
    & Dist$_y$  & - & - & 0.0020 (0.002) & 0.0048 (0.009) & 0.0050 (0.005) & 0.0015 (0.002) & 0.0011 (0.001) & \textbf{0.0010} (0.002) \\
    & Dist$_{xy}$  & - & - & 0.0030 (0.003) & 0.0053 (0.009) & 0.0044 (0.005) & 0.0025 (0.002) & \textbf{0.0013} (0.001) & 0.0021 (0.003) \\
\midrule
    Diabetes & MAE$_z$  & 46.258 (29.401) & - & 36.490 (5.383) & 42.440 (31.524) & 34.825 (37.760) & 9.7601 (2.963) & 15.162 (9.132) & \textbf{7.6517} (4.250) \\
    & MAE$_x$ & 0.9694 (0.140) & - & 0.9694 (0.140) & 2.3214 (0.390) & 1.0867 (0.091) & - & \textbf{0.9541} (0.128) & 0.9643 (0.136) \\
    & PCC & 0.3495 (0.139) & - & 0.3025 (0.039) & 0.3687 (0.148) & 0.4743 (0.204) & 0.6248 (0.081) & 0.5715 (0.109) & \textbf{0.6948} (0.114) \\
    & Dice & 0.9028 (0.019) & - & 0.9028 (0.019) & 0.7489 (0.070) & 0.8909 (0.016) & - & \textbf{0.9060} (0.018) & 0.9039 (0.018) \\
    & Curv$_x$  & 1.0007 (0.001) & 1.0007 (0.001) & 1.0000 (0.000) & \textbf{1.0007} (0.001) & \textbf{1.0007} (0.001) & \textbf{1.0007} (0.001) & \textbf{1.0007} (0.001) & \textbf{1.0007} (0.001) \\
    & Dist$_x$  & - & - & 0.0007 (0.001) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) \\
    & Curv$_y$  & - & 1.0005 (0.000) & 1.0000 (0.000) & 1.0079 (0.007) & 1.0091 (0.013) & 1.0000 (0.000) & 1.0023 (0.002) & \textbf{1.0006} (0.000) \\
    & Dist$_y$  & - & - & 0.0005 (0.000) & 0.0075 (0.007) & 0.0090 (0.012) & 0.0004 (0.000) & 0.0018 (0.001) & \textbf{0.0003} (0.000) \\
    & Dist$_{xy}$  & - & - & 0.0007 (0.001) & 0.0073 (0.006) & 0.0086 (0.012) & 0.0006 (0.001) & 0.0019 (0.001) & \textbf{0.0004} (0.000) \\
\midrule
    ERM & MAE$_z$  & 22.952 (2.705) & - & 25.456 (0.886) & 18.859 (1.030) & 17.515 (2.854) & 6.9292 (5.139) & 9.3311 (2.225) & \textbf{5.3988} (1.212) \\
    & MAE$_x$ & 0.9388 (0.000) & - & 0.9388 (0.000) & 1.4898 (0.286) & 0.9490 (0.010) & - & \textbf{0.9184} (0.020) & \textbf{0.9184} (0.020) \\
    & PCC & 0.4793 (0.026) & - & 0.3786 (0.005) & 0.4950 (0.016) & 0.5174 (0.035) & 0.7210 (0.146) & 0.6510 (0.066) & \textbf{0.7694} (0.012) \\
    & Dice & 0.8993 (0.010) & - & 0.8993 (0.010) & 0.8029 (0.074) & 0.8990 (0.011) & - & \textbf{0.9017} (0.007) & \textbf{0.9017} (0.007) \\
    & Curv$_x$  & 1.0002 (0.000) & 1.0002 (0.000) & 1.0000 (0.000) & \textbf{1.0002} (0.000) & \textbf{1.0002} (0.000) & \textbf{1.0002} (0.000) & \textbf{1.0002} (0.000) & \textbf{1.0002} (0.000) \\
    & Dist$_x$  & - & - & 0.0002 (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) \\
    & Curv$_y$  & - & 1.0003 (0.000) & 1.0000 (0.000) & 1.0038 (0.003) & 1.0040 (0.003) & \textbf{1.0001} (0.000) & 1.0013 (0.000) & 1.0007 (0.001) \\
    & Dist$_y$  & - & - & 0.0003 (0.000) & 0.0035 (0.003) & 0.0037 (0.003) & \textbf{0.0003} (0.000) & 0.0010 (0.000) & 0.0004 (0.000) \\
    & Dist$_{xy}$  & - & - & 0.0002 (0.000) & 0.0036 (0.002) & 0.0038 (0.003) & \textbf{0.0001} (0.000) & 0.0011 (0.000) & 0.0007 (0.001) \\
\midrule
    Other & MAE$_z$  & 24.536 (4.740) & - & 49.170 (1.546) & 19.713 (4.945) & 21.733 (4.834) & 18.388 (2.229) & 13.920 (7.803) & \textbf{6.3252} (3.322) \\
    & MAE$_x$ & 1.0408 (0.245) & - & \textbf{1.0408} (0.245) & 2.1735 (0.173) & 1.1122 (0.235) & - & \textbf{1.0408} (0.245) & \textbf{1.0408} (0.245) \\
    & PCC & 0.5202 (0.013) & - & 0.3563 (0.007) & 0.5657 (0.007) & 0.5788 (0.053) & 0.5623 (0.038) & 0.6487 (0.096) & \textbf{0.7625} (0.085) \\
    & Dice & 0.8977 (0.006) & - & \textbf{0.8977} (0.006) & 0.7547 (0.045) & 0.8888 (0.006) & - & \textbf{0.8977} (0.006) & \textbf{0.8977} (0.006) \\
    & Curv$_x$  & 1.0019 (0.000) & 1.0019 (0.000) & 1.0000 (0.000) & \textbf{1.0019} (0.000) & \textbf{1.0019} (0.000) & \textbf{1.0019} (0.000) & \textbf{1.0019} (0.000) & \textbf{1.0019} (0.000) \\
    & Dist$_x$  & - & - & 0.0019 (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) \\
    & Curv$_y$  & - & 1.0013 (0.000) & 1.0000 (0.000) & 1.0125 (0.007) & 1.0046 (0.003) & 1.0000 (0.000) & \textbf{1.0015} (0.001) & 1.0008 (0.000) \\
    & Dist$_y$  & - & - & 0.0013 (0.000) & 0.0112 (0.007) & 0.0033 (0.003) & 0.0013 (0.000) & \textbf{0.0004} (0.000) & 0.0005 (0.000) \\
    & Dist$_{xy}$  & - & - & 0.0019 (0.000) & 0.0106 (0.007) & 0.0031 (0.003) & 0.0019 (0.000) & \textbf{0.0007} (0.000) & 0.0011 (0.000) \\
\midrule
    Normal & MAE$_z$  & 11.494 (8.603) & - & 34.674 (13.856) & 10.878 (8.487) & 16.219 (16.053) & 10.864 (7.048) & 7.9207 (4.214) & \textbf{5.7582} (2.287) \\
    & MAE$_x$ & 0.2712 (0.378) & - & 0.2712 (0.378) & 1.4260 (0.554) & 0.3807 (0.344) & - & 0.2711 (0.364) & \textbf{0.2649} (0.360) \\
    & PCC & 0.6379 (0.129) & - & 0.3507 (0.087) & 0.6451 (0.129) & 0.5891 (0.168) & 0.6556 (0.164) & 0.6925 (0.100) & \textbf{0.7524} (0.080) \\
    & Dice & 0.9715 (0.039) & - & 0.9715 (0.039) & 0.7990 (0.066) & 0.9580 (0.037) & - & 0.9715 (0.038) & \textbf{0.9725} (0.037) \\
    & Curv$_x$  & 1.0014 (0.001) & 1.0014 (0.001) & 1.0000 (0.000) & \textbf{1.0014} (0.001) & \textbf{1.0014} (0.001) & \textbf{1.0014} (0.001) & \textbf{1.0014} (0.001) & \textbf{1.0014} (0.001) \\
    & Dist$_x$  & - & - & 0.0014 (0.001) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) & \textbf{0.0000} (0.000) \\
    & Curv$_y$  & - & 1.0007 (0.001) & 1.0000 (0.000) & 1.0015 (0.002) & 1.0021 (0.006) & 1.0001 (0.000) & \textbf{1.0006} (0.001) & \textbf{1.0006} (0.000) \\
    & Dist$_y$  & - & - & 0.0007 (0.001) & 0.0009 (0.002) & 0.0023 (0.006) & 0.0007 (0.001) & 0.0005 (0.001) & \textbf{0.0003} (0.000) \\
    & Dist$_{xy}$  & - & - & 0.0014 (0.001) & 0.0015 (0.002) & 0.0029 (0.006) & 0.0013 (0.001) & \textbf{0.0009} (0.001) & 0.0010 (0.001) \\
    
    \bottomrule
    \end{tabular*}
    \label{tab:disease_hv}
\end{table*}

==> tables/disease_stats.tex <==
% hv dataset
\begin{table}[htb]
% \tabcolsep=0.11cm
    \caption{Statistics of diseases in the two datasets.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
        Disease & Horizontal + Vertical Dataset & Horizontal Dataset  \\
    \midrule % GT
        wet AMD
        & 23
        &
        \\
    
        Dry AMD
        & 12
        &
        \\
        
        Diabetes
        & 9
        & 
        \\
        
        % ERM
        % & 11
        % &
        % \\
        
        Other
        & 40
        &
        \\
        
        Normal
        & 15
        &
        \\
        
    \bottomrule
    \end{tabular}
    \label{tab:disease_stats}
\end{table}

==> tables/moco_z_x.tex <==

% x motion result
\begin{table*}[htb]
% \tabcolsep=0.11cm
    \caption{Evaluation of different X motion correction networks on the test set.}
    \centering
    \fontsize{7.8}{9}\selectfont
    \begin{tabular}{lc@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{\hskip6pt}c@{}}
    \toprule
         & \multicolumn{7}{c}{Z correction only} & \multicolumn{3}{c}{GT Z correction + X correction only} \\
        \cmidrule(lr){3-8}
        \cmidrule(lr){9-11}
        \multicolumn{2}{@{}l}{Method} & $\mathrm{MAE_z}$ & PCC & $\mathrm{Curv}_x$ & $\mathrm{Dist}_x$ & $\mathrm{Curv}_y$ & $\mathrm{Dist}_y$ & $\mathrm{Dist}_{xy}$ & MAE$_x$ & PCC & Dice\\
    \midrule % GT
        \multicolumn{2}{@{}l}{No correction}
        & 0.7484 (0.4487) & 0.5505 (0.1492) & 0.9205 (0.0506)
        & 0.7484 (0.4487) & 0.9714 (0.0190) & 0.9205 (0.0506)
        \\
        
        \multicolumn{2}{@{}l}{Ground truth}
        & - & 1.000 (0.000) & 1.000 (0.000)
        & - & 1.000 (0.000) & 1.000 (0.000)
        \\
        
    \midrule % methods
        \multicolumn{2}{@{}l}{Antony et al. \cite{antony2011automated}}
        & 19.390 (11.521) & 0.595 (0.034)  & 0.869 (0.028)
        & 0.7484 (0.4487) & 0.9714 (0.0190) & 0.9205 (0.0506)
        \\
        
        \multicolumn{2}{@{}l}{Montuoro et al. \cite{montuoro2014motion}}
        & 1.8507 (0.5444) & 0.5635 (0.1509) & 0.7995 (0.0684)
        & 1.6152 (0.4604) & 0.9506 (0.0148) & 0.8191 (0.0564)
        \\
        
        \multicolumn{2}{@{}l}{Fu et al. \cite{fu2016eye}}
        & 0.8232 (0.4138) & 0.5604 (0.1401) & 0.9119 (0.0463)
        & 0.8185 (0.4375) & 0.9693 (0.0187) & 0.9127 (0.0494)
        \\
        
        \multicolumn{2}{@{}l}{Spectralis \cite{teussink2019spectralis}}
        & - & 0.6043 (0.1410) & -
        & - & - & -
        \\
        
    \midrule % method
    
        \multirow{2}{*}{Ours (baseline)} 
        & -
        & 13.948 (10.833)
        & 0.6185 (0.1124)
        & 1.0017 (0.0016)
        & 0.0007 (0.0014)
        & \textbf{1.0013} (0.0015)
        & 0.0009 (0.0011)
        & 0.0013 (0.0014)
        & \multirow{4}{*}{\textbf{0.7406} (0.4369)} & \multirow{4}{*}{\textbf{0.9716} (0.0187)} & \multirow{4}{*}{\textbf{0.9218} (0.0484)}
        \\
        
        & LS
        & 12.720 (9.504)
        & 0.6388 (0.1139)
        & \textbf{1.0020} (0.0023)
        & \textbf{0.0000} (0.0000)
        & 1.0016 (0.0018)
        & 0.0009 (0.0011)
        & \textbf{0.0012} (0.0012)
        \\
        
       \multirow{2}{*}{Ours (with seg.)}
        & -
        & 9.102 (7.972)
        & 0.7150 (0.0965)
        & 1.0012 (0.0012)
        & 0.0009 (0.0018)
        & 1.0009 (0.0005)
        & 0.0008 (0.0013)
        & 0.0015 (0.0021)
        \\
        
        & LS
        & \textbf{8.512} (8.211)
        & \textbf{0.7277} (0.1107)
        & \textbf{1.0020} (0.0023)
        & \textbf{0.0000} (0.0000)
        & 1.0008 (0.0005)
        & \textbf{0.0006} (0.0012)
        & 0.0014 (0.0019)
        \\
        
        % Ours (baseline)
        % & 0.7428 (0.4393) & 0.6388 (0.1139) & 0.9214 (0.0488)
        % & \multirow{2}{*}{\textbf{0.7406} (0.4369)} & \multirow{2}{*}{\textbf{0.9716} (0.0187)} & \multirow{2}{*}{\textbf{0.9218} (0.0484)}
        % \\
        
        % Ours (with seg.)
        % & \textbf{0.7401} (0.4404) & \textbf{0.7277} (0.1107) & \textbf{0.9219} (0.0490)
        % \\
        
    \bottomrule
    \end{tabular}
    \label{tab:moco_x}
\end{table*}


==> tables/new_data_stats.tex <==
% stats of new dataset
\begin{table}[htb]
% \tabcolsep=0.11cm
    \caption{Statistics of OCT resolution in horizontal dataset.}
    \centering
    \begin{tabular}{lcccc}
    \toprule
        Resolution & Count \\
    \midrule % GT
        $496\times 512\times 49$
        & 95
        \\
    
        % $496\times 512\times 15$
        % & 1
        % \\
        
        $496\times 512\times 25$
        & 3
        \\
        
        $496\times 1024\times 97$
        & 6
        \\
        
        $496\times 1024\times 49$
        & 2
        \\
        
    \bottomrule
    \end{tabular}
    \label{tab:new_data_stats}
\end{table}
